Real Time Cluster Path Tracing

Photorealistic rendering effects are common in films, but most real time graphics today still rely on scan-line based multi-pass rendering to deliver rich visual experiences. While there have been prior works in distributed path tracing for static scene and objects under rigid motion, real time path tracing of deforming characters has to support per-frame dynamic BVH changes. We present the architecture and implementation of the first real-time production quality cluster path tracing renderer that supports film quality animation and deformation. We build our cluster path tracing system using the open source Blender and its GPU accelerated production quality renderer Cycles. Our system's rendering performance and quality scales linearly with the number of RTX cluster nodes used. It is able to generate and deliver path traced images with global illumination effects to remote light-weight client systems at 15-30 frames per second for a variety of Blender scenes including animated digital human characters with skin deformation and virtual objects.

==> makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
    cluster_pt.tex \
	supplemental.tex


PDF = ${SAMPLES:%.tex=%.pdf} 

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


%.cls:   %.ins %.dtx
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


cluster_pt.pdf : introduction.tex \
           related.tex \
           realtime.tex\
           cluster.tex\
           results.tex\
           cluster_pt.bib

supplemental.pdf: supplemental.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi *.pdf

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf sample-*.pdf *.cls *.bst


==> perfstats_complete.tex <==
%\begin{figure}
\begin{table}[ht]
\begin{tabular}{|c|ccc|ccc|}
\hline
Scene &\multicolumn{3}{c|}{Tesla} & 
\multicolumn{3}{c|}{Trudy}  \\
%\hline
%Image Resolution&\multicolumn{6}{c|}{1280x720} \\
\hline
Working Nodes & 1& 2 & 5 & 1 & 5 & 10 \\
\hline
Working GPUs  & 10& 20 & 50 & 10 & 50 & 100 \\
\hline
Per Node SPP & 30 & 15 & 6 & 10 & 10 & 10 \\
\hline
Total  SPP 	& 30 & 30  & 30 & 10 &50 & 100 \\
\hline
Client FPS  & 7 &  15 & 27 & 14 & 14 & 14 \\
\hline
Timing Breakdown & \multicolumn{6}{c|} {ms} \\
\hline
Master render & 116.3 & 60.9 & 32.6  &29.9 &  29.5 & 29.9\\
Worker render  & n/a & 59.1 & 26.4 & n/a& 34.0 & 39.5\\
Master scene update  & 0.6& 1.2 & 1.0 & 36.2 & 33.2 & 33.4\\
Worker scene update  & n/a & 0.8 & 0.8 & n/a &31.2 & 29.2\\
Master update + render & 116.9  & 62.1 & 33.6 & 66.1& 62.7 & 64.3\\
Worker update + render & n/a  & 59.9 & 27.2 &n/a & 65.2 & 68.7\\
Master tone mapping & 2.1  & 2.0 & 2.0 & 2.0 & 1.6 & 1.6 \\
Master compression & 8.7 & 8.9 & 8.6 & 12.1 & 11.5 & 9.3\\
Master denoising & 14.5 & 14.7 & 13.9 & 0 & 0  & 0\\
%Master work distribution & 2.1 & 2.2 & 2.1 & 2.5 \\
%Master work merge & 3.3 & 3.5  & 3.2 & 3.7\\
%Master distribution $+$ merge   & 5.4 & 5.7 & 5.1 & 6.2\\ 
\hline
\end{tabular}
\caption {Performance measurements for real-time rendering of Tesla using $2$ and $5$ 
cluster nodes, and of Trudy using $5$ and $10$ cluster nodes.}
\label{fig:perf_stats}
\end{table}
\vspace{-2em}

